Efficient and Consistent Robust Time Series Analysis

We study the problem of robust time series analysis under the standard auto-regressive (AR) time series model in the presence of arbitrary outliers. We devise an efficient hard thresholding based algorithm which can obtain a consistent estimate of the optimal AR model despite a large fraction of the time series points being corrupted. Our algorithm alternately estimates the corrupted set of points and the model parameters, and is inspired by recent advances in robust regression and hard-thresholding methods. However, a direct application of existing techniques is hindered by a critical difference in the time-series domain: each point is correlated with all previous points rendering existing tools inapplicable directly. We show how to overcome this hurdle using novel proof techniques. Using our techniques, we are also able to provide the first efficient and provably consistent estimator for the robust regression problem where a standard linear observation model with white additive noise is corrupted arbitrarily. We illustrate our methods on synthetic datasets and show that our methods indeed are able to consistently recover the optimal parameters despite a large fraction of points being corrupted.

==> scratch.tex <==
\begin{lemma}
\label{lem:expectation}
Let $\vx \sim \cN(\vzero,I_{d \times d})$ and $g \sim N(0,\sigma^2)$ be two independently sampled random variables and let $\vla \in \bR^d$ be a fixed vector such that $\norm{\vla}_2 \leq \frac{\sigma}{100}$. Let $y = \vx^\top\vla + g$. Then for any $\tau > 0$, we have $\E{\ind{\abs{y} > \tau}\cdot y\cdot\vx} = C_\tau D^{-3}\vla$, where $D = \br{I + \frac{\vla\vla^\top}{\sigma^2}}^{1/2}$ and $C_\tau \leq 2.001\frac{1}{\sigma\sqrt{2\pi}}\cdot\br{\tau + \frac{1}{\tau}}\exp\br{-\frac{\tau^2}{2.001\sigma^2}}$.
\end{lemma}
\begin{proof}
Note that $y|\vx \sim \cN(\vx^\top\vla,\sigma^2)$. Letting $z = \ind{\abs{y} > \tau}\cdot y$ lets us write
\[
\E{z\cdot\vx} = \int_{\bR\backslash[-\tau,\tau]}\int_{\bR^d}y\cdot\vx\ p(\vx,y)\ d\vx\ dy.
\]
Let $D = \br{I + \frac{\vla\vla^\top}{\sigma^2}}^{1/2}$. Then for any fixed $y$, we have
\begin{align*}
\int_{\bR^d}y\cdot\vx\ p(\vx,y)\ d\vx &= \int_{\bR^d}y\cdot\vx\ p(\vx)p(y|\vx)\ d\vx\\
																			&= \frac{1}{\sigma(\sqrt{2\pi})^{d+1}}\int_{\bR^d}y\cdot\vx\ \exp\br{-\frac{\norm{\vx}_2^2}{2}} \exp\br{-\frac{(y - \vx^\top\vla)^2}{2\sigma^2}}\ d\vx\\
																			&= \frac{yD^{-2}}{\sigma(\sqrt{2\pi})^{d+1}}\int_{\bR^d}\vu\ \exp\br{-\frac{\norm{\vu}_2^2}{2} + \frac{y^2}{\sigma^2} - \frac{2y\vu^\top D^{-1}\vla}{\sigma^2}} \ d\vu\\
																			&= \frac{yD^{-2}\exp\br{-\frac{y^2}{2\sigma^2} + \frac{y^2\vla^\top D^{-2}\vla}{2\sigma^4}}}{\sigma(\sqrt{2\pi})^{d+1}}\int_{\bR^d}\vu\ \exp\br{-\frac{1}{2}\norm{\vu - \frac{yD^{-1}\vla}{\sigma^2}}_2^2} \ d\vu\\
																			&= \frac{y^2D^{-3}\vla\exp\br{-\frac{y^2}{2\sigma^2} + \frac{y^2\vla^\top D^{-2}\vla}{2\sigma^4}}}{\sigma^3\sqrt{2\pi}},
\end{align*}
where in the third step, we perform a change of variables $\vu = D\vx$. Plugging this into the expression for $\E{z\cdot\vx}$, invoking the guarantee of the coarse convergence analysis to ensure $\vla^\top D^{-2}\vla \leq \norm{\vla}_2 \leq \frac{\sigma}{100}$, and using elementary manipulations such as integration by parts gives us
\[
\E{\ind{\abs{y} > \tau}\cdot y\cdot\vx} = C_\tau D^{-3}\vla,
\]
where $C_\tau \leq 2.001\frac{1}{\sigma\sqrt{2\pi}}\cdot\br{\tau + \frac{1}{\tau}}\exp\br{-\frac{\tau^2}{2.001\sigma^2}}$ as claimed.
\end{proof}


\subsection{Innovational Corruptions}
Now consider the following innovational corruption mechanism (at most $\ko$ of $\bo_t$'s are non-zero):
\[
\vy_t ~=~ \vy_{t-1} \wo_1 + \ldots + \vy_{t-d} \wo_d + (\veps_t + \bo_t) \text{ for } i=1,\ldots,n.
\]
Then the innovationally corrupted time series observation $(y_{-d+1},\ldots,y_0,y_1,\ldots,y_n)$ can be modeled as follows
\begin{align}
\begin{bmatrix}
y_{1} \\
\vdots \\
y_{n}
\end{bmatrix}
~=~&
\begin{bmatrix}
y_0 & \cdots & y_{-d+1} \\
\vdots & & \vdots \\
y_{n-1} & \cdots & y_{n-d}
\end{bmatrix}
\cdot
\begin{bmatrix}
\wo_1 \\
\vdots \\
\wo_d
\end{bmatrix}
+
\begin{bmatrix}
\veps_{1} \\
\vdots \\
\veps_{n}
\end{bmatrix}
+
\begin{bmatrix}
\bo_{1} \\
\vdots \\
\bo_{n}
\end{bmatrix} \nonumber
\\
\vy ~=~& \bar{X}^\top \wo + \veps + \bo , \label{innovation-corruption-ar-d-actual-model}
\end{align}
where $\bo$ is $\ko$-sparse.

Thus our goal is to recover a parameter vector $\wo$, and to this end, we look to solve the following (non-convex) constrained problem 
\begin{equation}
\label{intermediate-non-cvx-objective-io}
\br{\hat{\vw},\hat{\vb}} = \argmin_{\vw,\vb} g(\vw,\vb) ~:=~ \frac{1}{2} \norm{\vy - \bar{X}^\top \vw - \vb}_2^2 \text{ s.t. } \norm{\vb}_0 \leq k,
\end{equation}
where $k \geq \ko$. The optimal value of $\vw$ that minimizes the above objective function w.r.t. $\vb$ is given as follows
\begin{equation}
\hat{\vw} ~=~ (\bar{X}\bar{X}^\top)^{-1} \bar{X}(\vy-\vb) .
\end{equation}
By substituting the above expression for $\vw$ in \eqref{intermediate-non-cvx-objective-io}, we get the resulting objective as follows 
\begin{align}
\label{final-non-cvx-objective-io}
\hat{\vb} = \argmin_{\vb} f(\vb) ~:=~ \frac{1}{2} \norm{(I- \bar{X}^\top (\bar{X}\bar{X}^\top)^{-1} \bar{X})(\vy-\vb)}_2^2 \text{ s.t. } \norm{\vb}_0 \leq k.
\end{align}
Since the gradient of $f(\vb)$ is $\nabla f(\vb) = (I- \bar{X}^\top (\bar{X}\bar{X}^\top)^{-1} \bar{X})(\vb-\vy)$, the constrained optimization problem \eqref{final-non-cvx-objective-io} can be solved using the iterative hard thresholding method as follows
\begin{align*}
\btn ~=~& \HT_k (\bt - \nabla f(\bt)) \\
~=~& \HT_k (\bt + (I- \bar{X}^\top (\bar{X}\bar{X}^\top)^{-1} \bar{X})(\vy-\bt)). 
\end{align*}


\begin{algorithm}[t]
	\caption{\small \ioard: Consistent Time Series Estimation with Innovational Outliers}
	\label{algo:ioard}
	\begin{algorithmic}[1]
		\small{
			\REQUIRE Time-series data $y_i, i=-d+1,\ldots,n$, thresholding parameter $k$, tolerance $\epsilon$, order of the time-series $d$
			\STATE $\vx_i \< (y_{i-1},\ldots,y_{i-d})^\top$, $\bar{X} \< \bs{\vx_1,\ldots,\vx_n}$, $\vy \< \br{y_1,\ldots,y_n}^\top$, $P_{\bar{X}} \< \bar{X}^\top (\bar{X}\bar{X}^\top)^{-1} \bar{X}$, $t \< 0$, $\vb^0 \< 0$, $\vr^0 \< \vy$
			\WHILE{$\norm{\vr^t}_2 \geq \epsilon$}
			\STATE $\btn \< \HT_k \br{P_{\bar{X}} \bt + \br{I - P_{\bar{X}}} \vy}$
			\STATE $\wtn \< \br{\bar{X}\bar{X}^\top}^{-1} \bar{X} \br{\vy-\btn}$
			\STATE $r^{t+1} \< ((\vy-\btn)-\bar{X}^\top \wtn)$
			\STATE $t \< t+1$
			\ENDWHILE
			\STATE \textbf{return} $\wt$
		}
	\end{algorithmic}
\end{algorithm}

\subsubsection{Restricted Singular values of $X$}

\begin{theorem}
	\label{clean-sssc-ssss}
	Let $X$ be a matrix whose columns are sampled from a stationary and stable $\VAR$ process given by \eqref{var-modify} i.e. $X_i \sim \cN\br{0,C_X}$. Then for any $k \leq n$, with probability at least $1-\delta$, the matrix $X$ satisfies the SSSC and SSSS properties with constants
	\begin{align*}
	\Lambda_k ~\leq~& k \bc{ \cM_{\yo} + \sqrt{ \cM_{\uo} \cM_{\yo} \frac{1}{c} \log{\frac{en}{k}}} + \cM_{\uo} \log{\frac{en}{k}}} \\
	& + \cO\br{\sqrt{k \alpha_2(d,\delta) \cM_{\uo} \cM_{\yo}}} + \cO\br{\alpha_2(d,\delta) \cM_{\uo}} &~=:~ U_k \\
	\lambda_k ~\geq~& n \mathfrak{m}_{\yo} - \br{n-k} \bc{ \cM_{\yo} + \sqrt{ \cM_{\uo} \cM_{\yo} \frac{1}{c} \log{\frac{en}{n-k}}} + \log{\frac{en}{n-k}} \cM_{\uo}} \\
	& - \Omega \br{\br{1+\sqrt{\frac{n-k}{n}}}\sqrt{n \alpha_2(d,\delta) \cM_{\uo} \cM_{\yo}}} - \Omega \br{\alpha_2(d,\delta) \cM_{\uo}} &~=:~ L_k ,
	\end{align*}
	where $\alpha_2(d,\delta)=\log{\frac{1}{\delta}} + d$ and $c$ is some universal constant.
\end{theorem}
\begin{proof}
	One can easily observe that considering the columns-restricted matrix $X_S$ wouldn't impact the analysis of Lemma~\ref{full-singular-values}. Thus for any fixed $S \in \cS_k$, Lemma~\ref{full-singular-values} guarantees the following bound (since $\abs{S}=k$)
	\begin{align*}
	\lambda_{\max}\br{X_S X_S^\top} ~\leq~& k \cM_{\yo} + (1-2\epsilon)^{-1} \bc{\sqrt{k \alpha_1(d,\delta,\epsilon) \cM_{\uo} \cM_{\yo}} + \alpha_1(d,\delta,\epsilon) \cM_{\uo}}.
	\end{align*}
	Taking a union bound over $\cS_k$ and noting that $\abs{\cS_k} \leq \br{\frac{en}{k}}^{k}$, gives us with probability at least $1-\delta$ 
	\[
	\Lambda_k ~\leq~ k \cM_{\yo} + (1-2\epsilon)^{-1} M,
	\]
	where
	\begin{align*}
	M ~=~& \sqrt{\br{\alpha_1 (d,\delta,\epsilon) + c k \log{\frac{en}{k}}} k \cM_{\uo} \cM_{\yo}} + \br{\alpha_1 (d,\delta,\epsilon) + c k \log{\frac{en}{k}}} \cM_{\uo} \\
	~\leq~& \sqrt{\alpha_1 (d,\delta,\epsilon) k \cM_{\uo} \cM_{\yo}} + k \sqrt{c \log{\frac{en}{k}} \cM_{\uo} \cM_{\yo}} + \br{\alpha_1 (d,\delta,\epsilon) + c k \log{\frac{en}{k}}} \cM_{\uo}.
	\end{align*}
	If $c<1$ (which can be ensured by scaling), by setting $\epsilon=\frac{1}{2} (1-c)$ and noting that $\Theta\br{\frac{1}{c} \alpha_1 \br{d,\delta,\frac{1-c}{2}}} = \Theta\br{\log{\frac{1}{\delta}} + d}$, we get
	\begin{align*}
	\Lambda_k ~\leq~& k \bc{\cM_{\yo} + \sqrt{\cM_{\uo} \cM_{\yo} \frac{1}{c} \log{\frac{en}{k}}} + \cM_{\uo} \log{\frac{en}{k}}} \\
	& + \cO\br{\sqrt{k \br{\log{\frac{1}{\delta}} + d} \cM_{\uo} \cM_{\yo}}} + \cO\br{\br{\log{\frac{1}{\delta}} + d} \cM_{\uo}}.
	\end{align*}
	For the second bound, we use the equality 
	\[
	X_S X_S^\top = X X^\top - X_{\bar{S}} X_{\bar{S}}^\top ,
	\]
	which provides the following bound for $\lambda_k$,
	\[
	\lambda_k ~\geq~ \lambda_{\min}\br{X X^\top} - \max_{T \in \cS_{n-k}} \lambda_{\max} \br{X_T X_T^\top} ~=~ \lambda_{\min}\br{X X^\top} - \Lambda_{n-k} .
	\] 
	Using Lemma~\ref{full-singular-values} to bound the first quantity and the first part of this theorem to bound the second quantity
	gives us, with probability at least $1-\delta$,
	\begin{align*}
	\lambda_k ~\geq~& n \mathfrak{m}_{\yo} - \br{n-k} \bc{\cM_{\yo} + (1-2\epsilon)^{-1} \br{\sqrt{c \log{\frac{en}{n-k}} \cM_{\uo} \cM_{\yo}} + c \log{\frac{en}{n-k}} \cM_{\uo}}} \\
	& - (1-2\epsilon)^{-1} \bc{\br{1+\sqrt{\frac{n-k}{n}}}\sqrt{n \alpha_1 (d,\delta,\epsilon) \cM_{\uo} \cM_{\yo}} + 2 \alpha_1 (d,\delta,\epsilon) \cM_{\uo}}.
	\end{align*}
	By setting $\epsilon=\frac{1}{2} (1-c)$ we get the following bound
	\begin{align*}
	\lambda_k ~\geq~& n \mathfrak{m}_{\yo} - \br{n-k} \bc{ \cM_{\yo} + \sqrt{ \cM_{\uo} \cM_{\yo} \frac{1}{c} \log{\frac{en}{n-k}}} + \log{\frac{en}{n-k}} \cM_{\uo}} \\
	& - \Omega \br{\br{1+\sqrt{\frac{n-k}{n}}}\sqrt{n \br{\log{\frac{1}{\delta}} + d} \cM_{\uo} \cM_{\yo}}} - \Omega \br{\br{\log{\frac{1}{\delta}} + d} \cM_{\uo}}.
	\end{align*}
\end{proof}


